Communication-free Massively Distributed Graph Generation

Analyzing massive complex networks yields promising insights about our everyday lives. Building scalable algorithms to do so is a challenging task that requires a careful analysis and an extensive evaluation. However, engineering such algorithms is often hindered by the scarcity of publicly~available~datasets. Network generators serve as a tool to alleviate this problem by providing synthetic instances with controllable parameters. However, many network generators fail to provide instances on a massive scale due to their sequential nature or resource constraints. Additionally, truly scalable network generators are few and often limited in their realism. In this work, we present novel generators for a variety of network models that are frequently used as benchmarks. By making use of pseudorandomization and divide-and-conquer schemes, our generators follow a communication-free paradigm. The resulting generators are thus embarrassingly parallel and have a near optimal scaling behavior. This allows us to generate instances of up to $2^{43}$ vertices and $2^{47}$ edges in less than 22 minutes on 32768 cores. Therefore, our generators allow new graph families to be used on an unprecedented scale.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> hyperbolic/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> hyperbolic/app-additional-results.tex <==
\section{Additional experimental results}
\begin{table}[h!]
	\begin{center}
		\input{results/table_compare.tex}
	\end{center}
	
	\vspace{2em}
	
	\caption{Comparison of generators for $n=2^{26}$, $\alpha \in \{0.55, 1\}$, and $\bar d \in \{10, 1000\}$.
		\textsl{Comp} refers to the number of distance computations between two points.
		It does not include node pairs that could be ruled out earlier (e.g., by comparing indices or radii).
		For \hypgen{} the value is higher due to vectorisation which often prevents such early discarding.
		\textsl{RSS} is the maximal resident set size (i.e. peak memory allocation) as reported by the operating system.
		In case of \rhg{} it is the sum of RSS of all MPI processes yielding a higher overhead.
		\girggen{} is a purely sequential implementation and includes fewer data points due to the high runtime.
		We report the standard deviation of the $S$ measurements as uncertainty and apply statistical error propagation.
		\\
		\vspace{0.5em}
		$\dagger$ Experiment was cancelled after a runtime of $10^5$~s.	
	}
	\label{tab:generator_compares}
\end{table}

\newcommand{\appScale}{0.63}

\begin{figure}
	\scalebox{\appScale}{\input{results/plot_gtime_d10_e21_abs.pgf}}
	\hfill
	\scalebox{\appScale}{\input{results/plot_gtime_d10_e21_rel.pgf}}

	\scalebox{\appScale}{\input{results/plot_gtime_d10_e30_abs.pgf}}
	\hfill
	\scalebox{\appScale}{\input{results/plot_gtime_d10_e30_rel.pgf}}

	\scalebox{\appScale}{\input{results/plot_gtime_d1000_e21_abs.pgf}}
	\hfill
	\scalebox{\appScale}{\input{results/plot_gtime_d1000_e21_rel.pgf}}

	\scalebox{\appScale}{\input{results/plot_gtime_d1000_e30_abs.pgf}}
	\hfill
	\scalebox{\appScale}{\input{results/plot_gtime_d1000_e30_rel.pgf}}
	
	\caption{Runtime of generators as function of the number $n$ of nodes.}
	\label{fig:runtimeofn}
\end{figure}

\begin{figure}
	\scalebox{\appScale}{\input{results/plot_ressize_d10_e21_abs.pgf}}
	\hfill
	\scalebox{\appScale}{\input{results/plot_ressize_d10_e21_rel.pgf}}
	
	\scalebox{\appScale}{\input{results/plot_ressize_d10_e30_abs.pgf}}
	\hfill
	\scalebox{\appScale}{\input{results/plot_ressize_d10_e30_rel.pgf}}
	
	\scalebox{\appScale}{\input{results/plot_ressize_d1000_e21_abs.pgf}}
	\hfill
	\scalebox{\appScale}{\input{results/plot_ressize_d1000_e21_rel.pgf}}
	
	\scalebox{\appScale}{\input{results/plot_ressize_d1000_e30_abs.pgf}}
	\hfill
	\scalebox{\appScale}{\input{results/plot_ressize_d1000_e30_rel.pgf}}
	
	\caption{Max. memory allocation of generators as function of the number $n$ of nodes.}
	\label{fig:ressizeofn}
\end{figure}

==> hyperbolic/app-identities.tex <==
\section{Definitions, Useful Identities and Approximations}\label{sec:app-definitions}
\subsection{Hyperbolic Functions}
Hyperbolic functions:
\begin{align*}
  \sinh(x) &\defrel \frac 1 2 \left( e^{x} - e^{-x} \right) \\
  \cosh(x) &\defrel \frac 1 2 \left( e^{x} + e^{-x} \right) \\ \\
  \intertext{Inverse hyperbolic functions:}
  \asinh(y) &= x \ \Rightarrow\ \sinh(x) = y \\
  \acosh(y) &= x \ \Rightarrow\ \cosh(x) = y
\end{align*}

\subsection{Geometry Related Definitions}
Radial density:
\begin{align*}
	\rho(r) &\defrel \alpha \frac{\alpha \sinh(\alpha r)}{\cosh(\alpha R)}
  \intertext{Radial cdf:}
	\mu(B_r(0)) &\defrel \int_{0}^{r} \rho(x) \intd x = \frac{\cosh(\alpha x) - 1}{\cosh(\alpha R)} 
  \intertext{Angular deviation:}
	\Delta\theta(r, b) &\defrel 
	\begin{cases}
		\pi & \text{if } r{+}b < R \\
		\arccos\big[\frac{\cosh(r)\cosh(b) - \cosh(R)}{\sinh(r)\sinh(b)}\big] & \text{otherwise}
	\end{cases}
\end{align*}

\vspace{1em}

\subsection{Approximations}
Gugelmann et al. derived the following approximations\footnote{We drop the $(1 + \Oh(\cdot))$ error terms in our calculations without further notice if they are either irrelevant or dominated by other simplifications made}~\cite{DBLP:conf/icalp/GugelmannPP12}.\\

\noindent Angular deviation:
\begin{align}\label{eq:deltathetaapprox}
	\Delta\theta(r, b) &= 
	\begin{cases}
	\pi & \text{if } r+b < R \\
	2\e^\frac{R-r-y}{2} (1 + \Theta(e^{R-r-y})) & \text{if } r+b \ge R
	\end{cases}\\	
\intertext{Radial cdf:}\label{eq:cdf}
	\mu(B_r(0)) 
		&= \int^{r}_{0} \rho(x) \intd x 
    = \frac{\cosh(\alpha r)}{\cosh(\alpha R) - 1} \\
    &= \e^{\alpha(r-R)} (1 + o(1)) 
\end{align}


==> hyperbolic/app-speedup.tex <==
\begin{table}
\scalebox{0.8}{
\begin{tabular}{|l||r|r||r|r||r|r||r|r|}
	\hline
	& \multicolumn{2}{c||}{$\bar d {=} 10^1,\ \alpha{=}0.55$}& \multicolumn{2}{c||}{$\bar d {=} 10^1,\ \alpha{=}1$}& \multicolumn{2}{c||}{$\bar d {=} 10^3,\ \alpha{=}0.55$}& \multicolumn{2}{c|}{$\bar d {=} 10^3,\ \alpha{=}1$}\\\hline
	& {\footnotesize Time/edge} & {\footnotesize Speed-up}   & {\footnotesize Time/edge} & {\footnotesize Speed-up}   & {\footnotesize Time/edge} & {\footnotesize Speed-up}   & {\footnotesize Time/edge} & {\footnotesize Speed-up} \\\hline
	\nkgen 
	& $180.4 \pm 9.7$ & n/a
	& $178.0 \pm 11.6$ & n/a
	& $28.7 \pm 0.2$ & n/a
	& $78.9 \pm 0.1$ & n/a
	\\\hline
	\nkgenopt
	& $120.1 \pm 0.5$ & $1.5 \pm 0.0$
	& $116.6 \pm 6.2$ & $1.5 \pm 0.1$
	& $9.2 \pm 0.1$ & $3.1 \pm 0.0$
	& $7.7 \pm 0.0$ & $10.3 \pm 0.0$
	\\\hline
	\hypgen
	& $31.7 \pm 0.7$ & $5.7 \pm 0.1$
	& $44.3 \pm 2.5$ & $4.0 \pm 0.3$
	& $2.6 \pm 0.0$ & $10.8 \pm 0.2$
	& $2.7 \pm 0.0$ & $29.6 \pm 0.4$
	\\\hline
\end{tabular}}

\vspace{1em}

\caption{
	Runtime of \nkgen, \nkgenopt{} and \hypgen{} for $\alpha \in \{0.55, 1\}$ and $\bar d \in \{10, 1000\}$.
	The runtime per edge is reported in nanoseconds and computed as the total runtime divided by the number of edges produces.
	It is the average over all runs with $n \ge 10^8$.
	We report the standard deviation as uncertainty.
}
\label{tbl:speedup}
\end{table}

==> hyperbolic/conclusion.tex <==

In this paper, we presented our memory-efficient distributed memory graph generator for threshold random hyperbolic graphs.
Our novel algorithm combines divide-and-conquer schemes, an efficient partitioning of the hyperbolic space and a memory-efficient edge generation process.
In particular, we partition the hyperbolic space into a set of slabs and buckets using a divide and conquer algorithm proposed by Sanders~\etal~\cite{sanders2016efficient}.
We then traverse the resulting data-structure by using a memory-efficient request-centric approach and stream the resulting edges.
Additionally, our distributed algorithm focuses on scalability by using redundant computations instead of communication between PEs.
This is made possible by exploiting pseudorandomness via high-quality hash functions.
The resulting graph generator is communication-free, \ie~it requires no communication between different PEs at all.

Our extensive experimental evaluation indicates that our generator is outperforming both shared-memory and distributed-memory state-of-the-art algorithm.
In particular, we are up to $x$ times faster than the currently fastest shared-memory algorithm for a wide range of parameters.
Likewise, we are up to $y$ times faster than the distributed-memory algorithm \rhg while also providing a better scaling behavior.
This allows us to generate instances of up to $2^{x}$ vertices and $2^{y}$ edges in less than $z$ seconds on $32768$ PEs on the SuperMUC supercomputer.
To the best of our knowledge, these are the largest instances of threshold random hyperbolic graphs generated in practice.
These results enable random hyperbolic graphs to be used on massive scales by both algorithm developers and researchers alike.

Finally, we plan to generalize our approach for the probabilistic random hyperbolic graph model.
This would provide an even wider spectrum of realistic scale-free graph instances~\Todo{What else would be like to do?}.


==> hyperbolic/experiments.tex <==
A prototypical implementation of our graph generator (\rhgthres) in \CC~is available at \url{https://github.com/massive-graphs/RHGThres}. \Todo{Are you guys fine with putting it into the massive-graphs GitHub organization? We want to collect algo implementations without explicitly attributing it to a GitHub user.}


In this section, we compare our algorithm to existing state-of-the-art solutions in terms of (1) sequential performance, (2) shared-memory performance, and (3) distributed memory performance.
To be more specific, we compare our new algorithm \rhgthres to \hypgen~\cite{penschuck2017generating}, \nkgen~\cite{DBLP:conf/hpec/LoozOLM16}, \nkgenopt, \rhg~\cite{funke2017communication}, and \girggen~\cite{DBLP:journals/corr/BringmannKL15}.
With the exception of \girggen, all of these generators support shared-memory parallelism based on OpenMP.
Additionally, \rhgthres and \rhg also support distributed-memory parallelism based on MPI.
In fact, \rhgthres employs a hybrid design using both MPI and OpenMP allowing multiple compute nodes and the use of lightweight threads on a single node.

We now cover some implementation specifics for the individual algorithms that we use in our evaluation.
All algorithms and libraries are compiled using \GG~version 5.4.1 using optimization level \texttt{fast} and \texttt{-march=native}.
As an exception, \hypgen{} has to use a hardware-specific compiler, links against Intel's TBB malloc\_proxy, but otherwise has the same code basis as the CPU version.
In the distributed setting, we use Intel MPI~version 1.4 compiled with \GG~version 4.9.3.

Furthermore, our algorithm uses Spooky Hash\footnote{\url{http://www.burtleburtle.net/bob/hash/spooky.html}} as a hash function for pseudorandomization.
Hash values are used to initialize a Mersenne Twister~\cite{matsumoto1998mersenne} for generating uniform random deviates.
Binomial random deviates are generated using the \CC~standard library.

To fully exploit \rhgthres's on-the-fly edge generation, none of the implementations writes the edge list into memory.
We rather simulate a very simplistic streaming algorithm which consumes the edge stream and computes a fingerprint by summing all node indices contained.\footnote{We removed the appropriate memory allocations and accesses from \nkgen, \rhg, and \girggen, and added the streaming simulation.}
This choice enforces that the generators have to compute and forward every edge but does not impose memory restrictions.

\noindent
The runtime benchmarks were conducted on one of the following systems:
\begin{itemize}
	\item
		Indicated by {(Phi)}: 
    Intel Xeon Phi 5120D (60~cores, 240~threads, 1.05GHz),
		8~GB~GDDR5 RAM
		Linux~2.6.38,
		ICC~17.0.0,
		Intel TBB malloc\_proxy

	\item
		Indicated by {(CPU)}: 
		Intel Xeon CPU E5-2630~v3 (8~cores, 16 threads, 2.40GHz) with AVX2/SSE4.2 support for 4-way double-precision vectorisation,
		64~GB 2133~MHz RAM,
		Linux~4.8.1,
		GCC~6.2.1,
		VC (8. Dec. 2016),
		MPICH 3.2-7

	\item 
		Indicated by {(SuperMUC)}: 
    SuperMUC Phase 1 thin nodes (18 islands, total of 9216 compute nodes),
    two Sandy Bride-EP Xeon E5-2680 8C processors (16 cores per node), 
    32~GB~RAM~\Todo{add frequency},
    SUSE Linux Enterprise Server (SLES),
    GCC 4.9.3
    IntelMPI 1.4
\end{itemize}

\subsection{Shared-Memory Experiments}\label{subsec:exp-shared}

\subsection{Distributed-Memory Experiments}\label{subsec:exp-distributed}
In this section, we take at the look at the weak-/strong-scaling performance of our distributed generator.
Additionally, we compare its performance to the current state-of-the-art algorithm \rhg~\cite{funke2017communication}.
In particular, we are interested in the time required for generating massive instances of up to $2^{40}$ vertices with varying average degrees and power-law exponents.
As for Section~\ref{subsec:exp-shared}, we use average degrees ranging from $4$ to $256$ and power-law exponents from $2.2$ to $3.0$
These parameters ensure that we cover various extremes while keeping the resulting instances close to different real-world graphs~\cite{von2015fast}.
As mentioned in Section~\ref{subsec:par_thres}, a set of PEs if solely responsible for generating the inner clique of vertices with radius $r \leq \frac R 2$.
To fully exploit shared-memory parallelism, we dedicate a single compute node with $16$ PEs to this purpose.

We begin by examining the weak scaling behavior of our algorithm, \ie~the total running time over an increasing amount of PEs for a fixed number of vertices $n$ for each PE.
Figure~\ref{fig:rhgPar3} shows the weak scaling behavior for varying numbers of $n$, an average degree $d \in \{4, 64\}$ and a power-law exponent $\gamma = 3$.
First, we notice that there is a steep decrease in running time for the initial numbers of PEs for both average degrees.
This can be attributed to the introduction of streaming slabs and the exploitation of locality with an increase in the number of chunks.
Afterwards, the running time of our algorithm remains nearly constant until very large numbers of PEs.
Thus, we achieve a near-optimal scaling behavior.
Finally, for the largest numbers of PEs, the size of chunks shrinks and thus the number of global slabs is increased.
In turn, the degree of parallelism is reduced and we observe an increase in running time.
However, due to the particular choice of $\gamma = 3$ most vertices lie on the outside of the hyperbolic disk.
Thus this increase is rather small but more significant for larger average degrees.

If we decrease the power-law exponent sufficiently enough, the degree of parallelism of our partitioning becomes a bit more limited.
To illustrate this, Figure~\ref{fig:rhgPar22} shows the weak scaling behavior for varying numbers of $n$, an average degree $d \in \{4, 64\}$ and a power-law exponent $\gamma = 2.2$.
First, we notice that for lower average degrees, the initial scaling behavior is similar to larger power-law exponent.
However, since more and more vertices reside in the inner clique or lower global slabs, the degree of parallelism is quickly reduced.
In turn, we have a near-exponential increase in running time with an increasing number of PEs.
For larger average degrees, this effect is noticeable more quickly since the number of streaming slabs is further reduced.
This is due to the increase in the angular deviation for request with an increasing average degree.

Finally, we compare our algorithm to the state-of-the-art algorithm \rhg.
Figure~\ref{} shows the weak scaling behavior for both algorithm for varying numbers of $n$, an average degree $d \in \{4, 64\}$ and a power-law exponent $\gamma = 3$.
Additional plots for different choices of $\gamma$ can be seen in Appendix~\ref{}.
First, we are able to see that \rhgthres has both a better scaling behavior and an overall faster runtime.
To be more specific, \rhgthres is up to $x$ times faster than \rhg for smaller instances and up to $y$ times faster for the largest instances.
Additionally, the runtime of \rhgthres remains constant up to larger number of PEs, resulting in a better scaling behavior.
Finally, due to the optimized memory consumption, \rhgthres is able to generate significantly larger instances than its competitor.
To the best of our knowledge, we are able to generate the largest instances of hyperbolic random graphs currently available in practice.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.49\textwidth]{figures/plots/various_3_rhg_weak.pdf}
  \caption{\label{fig:rhgPar3}Running time for generating $nP$ vertices and an expected number of $mP=nP \cdot \bar{d}$ edges for varying $\bar{d}$ and a power-law exponent of $\gamma=3$ on $P$ PEs using \rhgthres.}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.49\textwidth]{figures/plots/various_22_rhg_weak.pdf}
  \caption{\label{fig:rhgPar22}Running time for generating $nP$ vertices and an expected number of $mP=nP \cdot \bar{d}$ edges for varying $\bar{d}$ and a power-law exponent $\gamma=2.2$ on $P$ PEs using \rhgthres.}
\end{figure}


==> hyperbolic/figures/request_point_inversion.tex <==
\begin{tikzpicture}
	\newcommand{\request}[4]{
		\path[draw, |-|] (#1, #2) to + (2*#3, 0);
		\node at (#1+#3, #2) {$\times$};
%		\node[anchor=north west] at (#1, #2) {\footnotesize $\theta_{#4}$};
	}

	\def\bwidth{10}
	
	\path[draw, <->] (0, 2.5) to (0, -.5) to (\bwidth + 0.5, -.5);
	\node[anchor=east] at (-0.1, 2.5) {$r$};
	\node[anchor=west] at (\bwidth + 0.6, -0.5) {$\theta$};
	
	\path[draw, dashed] (-0.1, 2) to (\bwidth, 2);
	\path[draw, dashed] (-0.1, 0) to (\bwidth, 0);
	
	\node[anchor=east] at (-0.1, 2) {$b_{i+1}$};
	\node[anchor=east] at (-0.1, 0) {$b_{i}$};
	
	\request{0.5}{0.2}{5}{i}
	\request{1.0}{0.6}{4}{i+1}
	\request{1.5}{1.0}{3}{i+2}
	\request{2.0}{1.4}{2}{i+3}
	\request{2.5}{1.8}{1}{i+4}
\end{tikzpicture}


==> hyperbolic/implementation.tex <==
\label{sec:implementation}
\subsection{Adjacency tests without trigonometric functions}\label{subsec:opt-trig}
The runtime of a preliminary version of our generator was dominated by repeated evaluations of trigonometric functions.
We address this issue with a pre-computing scheme.
Let $p = (r_p, \theta_p)$ and $q = (r_q, \theta_q)$ be two arbitrary points in $\mathcal{D}_R$ and let $\ell_i$ be the lower radial boundary of slab~$i$.

The scheme accelerates the two most frequent query types, namely the computation of request widths of form $\Delta\theta(r_p, \ell_i)$ and tests whether the hyperbolic distance $d(p, q) < R$ of two points falls below the threshold $R$.
The former computation type occurs $\Omega(n)$ times, while the latter is required in each of the $\Omega(m)$ candidate checks.
Based on Equation~\ref{eq:deltatheta} we obtain
\begin{multline}
	\Delta\theta(r_p, \ell_i) = \cos^{-1}\Big(\coth(r_p) \cdot \coth(\ell_i)\\
		- \frac{\cosh(R)}{\sinh(\ell_i)} \cdot \frac{1}{\sinh(r_p)} \Big),
\end{multline}
where $\coth(x) := \cosh(x) / \sinh(x)$.
By pre-computing $\coth(r_p)$ and $1 / \sinh(r_p)$ for each point, as well as $\coth(\ell_i)$ and $\cosh(R) / \sinh(\ell_i)$ for each slab, the argument of $\cos^{-1}$ follows from two multiplications and a subtraction.

Similarly, we test $d(p, q) < R$ by rewriting Equation~\ref{eq:hypdist}:
\begin{multline}
	\label{eq:effdistcomp}
	\cos(\theta_p)\cdot\cos(\theta_q) + \sin(\theta_p)\cdot\sin(\theta_q) < \\ 
	\coth(r_p) \cdot \coth(r_q) - \cosh(R) \cdot \frac{1}{\sinh(r_p)} \cdot \frac{1}{\sinh(r_q)},
\end{multline}
The left-hand-side is an expansion of $\cos(\theta_p - \theta_q)$.
Hence, the additional pre-computation of $\cos(\theta_p)$ and $\sin(\theta_p)$ for each point gives distance checks in at most five multiplications and two additions, which can be further improved by re-using parts of earlier computations.

Expression~\ref{eq:effdistcomp} can be vectorized efficiently and even allows for partially fused operations (cf. FMA instructions).
To support vectorized computations, we also use a structure-of-arrays memory layout to store active candidates.

\subsection{Batch-processing of requests}
{\rhgthres} effectively sweeps all slabs in an interleaved fashion and maintains for each slab a separate state containing the active candidates.
During this sweep, it encounters three event types, namely the occurrence of a point, the beginning of a request, and eventually its end.

Our implementation splits each slab into buckets of equal width and then processes these events batch-wise.
Given the number $n_j$ of points in slab~$j$, we select the number $c_j$ of buckets in slab~$j$ such that $c \le n_i / c_i < 2c$ where $c$ is a small tuning parameter (typically $8$).
More precisely, we choose $c_j$ as a power-of-two which by construction aligns cell boundaries between slabs and avoids corner cases when traversing the geometry.

When entering a bucket, we move all requests contained into the active state by first overwriting obsolete requests that went out-of-scope in the last bucket; we thereby avoid redundant operations otherwise caused by separated deletions and insertions.
Subsequently, all points contained are matched against the active candidates again increasing data locality and exploiting minor synergies.

The usage of buckets also allows us to relax the sorting of requests receive from below.
Rather than maintaining an exact order, a semi-sorting identify all requests starting/ending in the next bucket suffices.
Our implementations hence only stores for each request the indices of buckets in which it starts and ends, and orders the items in a radix heap.

While equidistant buckets allow for efficient index computations, they potentially cause a load imbalance\footnote{%
	Distributing points into buckets can be modeled as a ball into bins experiment.}.
The following lemma shows that this is asymptotically insignificant and thus confirms the speed-up observed in practice.

\begin{lemma}\label{lem:bucket-requests}
	Processing the requests within all buckets takes time $\Oh(n)$ in total with high probability.
\end{lemma}

\begin{proof}
	To bound the number of requests in a bucket we need take into account both requests from the bucket itself, as well as requests stemming from lower slabs.
	For this purpose, we first bound the number of requests stemming from a bucket itself.
	The number of points within a bucket follows a Poisson distribution with mean $\lambda = \frac n c$.
	Thus, the expected number of operations is $\expv{X^2} = \lambda^2 - \lambda = \Oh(1)$ and $\Oh(\log n)$ with high probability.
	However, since there are at most $\Oh(\frac{n}{\log n})$ buckets requiring $\Oh(\log n)$ operations, the amortized number of operations is linear.
	
	Next, we show that the number of operations stemming from requests from lower slabs is also linear in total.
	Following \ref{lem:candidates} and \ref{cor:candidates}, we observe that every point only gets an additional constant number of candidates more than the edges it produces.
	Additionally, we can (pessimistically) assume that every point gets a distinct set of candidates.
	Thus, the number of operations per bucket increases by an additional factor $X$ (number of points per bucket).
	Again, since $X=\Oh(\log n)$ with high probability for at most $\Oh(\frac{n}{\log n})$ buckets, the amortized number of operations is linear in total.
\end{proof}


==> hyperbolic/introduction.tex <==
\IEEEPARstart{R}{andom graph models} are an important tool to study the emergent properties and structures of artificial networks.
Models mimicking real-world graphs, such as social networks or the neural network of the human brain~\cite{Sporns2013}, are of special interest.
Common properties of these so-called \emph{complex networks} include a small diameter, non-vanishing clustering and a heavy-tailed degree distribution~\cite{DBLP:journals/corr/cond-mat-0106096, DBLP:conf/websci/BackstromBRUV12, DBLP:conf/www/MeuselVLB14, DBLP:conf/www/MyersSGL14}.
Gathering information about these networks is a crucial step to understand and algorithmically exploit their underlying structure.
  
Handling the huge amounts of data that are attributed to these massive systems requires algorithms that are capable of working on a petabyte scale.\Todo{Should we elaborate on that? cite?}
However, the design and evaluation of these algorithms is often hindered by the scarcity of publicly available datasets.\Todo{Might be interesting to include very large examples...?}

Models like the Recursive Matrix (R-MAT) model try to alleviate this problem by allowing to build massive synthetic instances with controllable parameters~\cite{DBLP:conf/sdm/ChakrabartiZF04}.
This makes them indispensable tools for high-performance computing benchmarks such as the Graph500~\cite{graph500}.
However, the degree of realism of the R-MAT model has been shown to be problematic for scaling studies~\cite{kolda2013scalable}.
\Todo{It might be interesting to also mention other distribution models (and point out limitation); could be done in related work as well}

Over recent years, geometric network models have gained increasing attention due to their natural resemblance to various types of networks networks.
In geometric networks a set of vertices is embedded in a geometric space and individual vertices are connected based on their distance.
Whereas Euclidean geometry has been shown to work well for modeling spatial networks such as ad-hoc wireless networks (e.g.,~\cite{DBLP:journals/tit/GuptaK00}), hyperbolic geometry provides a natural fit for complex scale-free networks~\cite{Sustaining2010, DBLP:journals/ton/ShavittT08}.
In particular, they have been shown to exhibit a small diameter, high clustering and a heavy-tailed power-law degree distribution~\cite{DBLP:conf/icalp/GugelmannPP12, DBLP:journals/corr/abs-1006-5169}.
Thus, much interest has been given to generating random hyperbolic graphs (RHGs) in a variety of different applications including graph partitioning~\cite{meyerhenke2017parallel}, machine learning~\cite{muscoloni2017machine} and routing~\cite{voitalov2017geohyperbolic}.

\subsection{Our contribution}
We propose a distributed random hyperbolic graph (RHG) generator that focus on scalability and memory efficiency.
Our algorithm {\rhgthres} uses the threshold model, {\ie} vertices are connected if and only if their distance is smaller than a given threshold value.
 
Our generator follows a communication-free paradigm, {\ie} it requires no communication between processing entities.
We achieve this property by making use of pseudorandomization via hash functions and an efficient decomposition of the hyperbolic plane.
In particular, we decompose the hyperbolic space into a set of slabs (concentric rings) that can be generated and traversed efficiently.
In turn, we are able to locally recompute parts of the network instead of using costly message exchanges.
Data locality and memory consumption are further improved using a request-centric streaming\footnote{%
	Vertices issue \textsl{edge requests} to neighbor candidates which may not have been sampled yet.}
approach that minimizes random I/O accesses.

The resulting generator is massively parallel and has a near optimal scaling behavior, both in terms of strong and weak scaling.
In particular, our algorithms achieve a time complexity of $\Oh(\frac{n \log \log n + m}{P} + P \log n + n^{1-\alpha}P^\alpha)$ and have a memory footprint of $\Oh()$~\todo{missing}.

Overall, we are able to generate instances of up to \Todo{$x$} vertices and \Todo{$y$} edges on \Todo{$z$} processors within \Todo{$w$} seconds.
These results compete with current graph generators used in high performance computing benchmarks such as the Graph500~\cite{graph500}.
%In turn, our results allow the RHG model to be fully utilized in a massively distributed setting.



==> hyperbolic/related_work.tex <==
\subsection{Random Hyperbolic Graph Model}\label{subsec:graph-model}
\begin{figure}[t]
  \centering
	{\adjustbox{trim={.25\width} {.245\height} {0.05\width} {.24\height},clip}{
		\scalebox{1}{\input{figures/hyperbolic_graph_model.pgf}}
	}}
	{\adjustbox{trim={.7\width} {.34\height} {0.0\width} {.34\height},clip}{
		\scalebox{0.8}{\input{figures/nkbands.pgf}}
	}}
	\caption{
		\textbf{Left}:
		The $G_{\alpha,C}(n)$ model with $n{=}150$, $\alpha{=}1$, $C{=}{-}2$.
		The area enclosed by each coloured lobe corresponds to all points in distance at most $R$ around its highlighted centre.
		\textbf{Right}: Band model introduced by \nkgen{} (not to scale).
		The partial blue lobe indicates the area in which candidates can be found.
		The step-wise overestimation for candidate selection is shown in yellow.
	}
	\label{fig:hyperbolic_model}
	\label{fig:band_overview}
	\vspace{-1em}
\end{figure}

Hyperbolic space (negative curvature) is one of the three isotropic spaces next to Euclidean (flat) and spherical space (positive curvature).
The crucial property of Hyperbolic geometry for modeling real world networks is its exponential expansion in space;
in particular, the area of a circle in the hyperbolic space grows exponentially with its radius.

Random hyperbolic graphs (RHGs) as a generative model were first introduced by Krioukov et al.~\cite{DBLP:journals/corr/abs-1006-5169}. 
To generate a graph in this model, points are distributed randomly on disk $\mathcal{D}_R$ with radius $R$ in the hyperbolic plane.
Each vertex $v_i$ is modeled as a point $p_i = (r_i, \theta_i)$ with a radial coordinate $r_i$ at an angle of $\theta_i$.
Its polar angle $\theta_i$ is drawn uniformly from the interval $[0, 2\pi)$ while its radial coordinate $0 \le r_i < R$ is governed by the density function 
\begin{equation}
  \label{eq:rho}
  \rho(r) = \frac{\alpha \sinh(\alpha r)}{\cosh(\alpha R) - 1}.
\end{equation}

Here, the parameter $\alpha$ describes the vertex dispersion. 
Vertex dispersion determines the power-law exponent of the degree distribution.
Intuitively, the smaller $\alpha$ the more likely are points with small radial components, which are expected to have a high number of neighbours.
The special case $\alpha = 1$ corresponds to the uniform distribution.
Krioukov et al.~\cite{DBLP:journals/corr/abs-1006-5169} showed that for $\alpha \geq \frac 1 2$ the resulting degree distribution follows a power-law with exponent $\gamma = 2\alpha + 1$.
% Furthermore, we assume $\alpha = \Oh(1)$ since real networks typically exhibit $2 \le \gamma \le 4$~(e.g., \cite{dorogovtsev2013evolution, DBLP:conf/kdd/KumarNT06}).

Vertices are connected by an edge with a probability governed by the density function $f_T(x)$ depending on the hyperbolic distance $x$ of the corresponding points and a temperature parameter $T \geq 0$:
\begin{equation}
  \label{eq:distprob}
  f_T(x) = \frac{1}{\exp(\frac{x-R}{2T}) + 1}
\end{equation}
The hyperbolic distance $d(p, q)$ between the two points $p = (r_p, \theta_p)$ and $q = (r_q, \theta_q)$ is given by
\begin{multline}
	\label{eq:hypdist}
	\cosh( d(p, q) ) = \cosh(r_p)\cosh(r_q) \\ - \sinh(r_p)\sinh(r_q)\cos(\theta_p - \theta_q).
\end{multline}

\subsection{Threshold Model $G_{\alpha,C}(n)$}
The threshold random hyperbolic graph model covers the special case of temperature $T=0$.
The significant difference to the standard model is that edges are now added between vertices if and only if their hyperbolic distance is below a given threshold.

Gugelmann et al.~\cite{DBLP:conf/icalp/GugelmannPP12} showed that this model is able to acurately describe the characteristics of many real-world networks including a high clustering and power-law degree distribution even up to the maximum degree. 
Additionally, they provide a set of approximations (including error terms) to simplify the analysis of the original model.
Their model, called $G_{\alpha,C}(n)$, forms the foundation of our work on threshold random hyperbolic graph generators.
The additional parameter $C$ controls the average degree $\bar d$ of the graph, which in turn is governed by:~\cite{DBLP:conf/icalp/GugelmannPP12}
\begin{equation}\label{eq:exp-deg}
	\expv{\, \bar d\,\,} = \frac 2 \pi \left( \frac{\alpha}{\alpha - 1/2} \right)^2 \e^{-C/2}
		 \errorterm{(1 + o(1))}
\end{equation}

\subsection{Random Hyperbolic Graph Generators}
Generating a random hyperbolic graph can be done na\"ively by computing the hyperbolic distance for all $\binom{n}{2}$ pairs of vertices.
Implementing this approach is possible with a constant memory overhead.
It is also trivially parallelizable;
the resulting generator however requires $\Theta(n^2)$ work on a \textsc{PRam}~\cite{JaJa92} rendering it infeasible for large graphs.

To reduce the number of vertex comparisons, most algorithms with sub-quadratic running time use a geometric decomposition of the hyperbolic space to identify a set of candidates $C(v) \subseteq V$ for each vertex $v \in V$.
Edges are then generated by performing distance computations between $v$ and $C(v)$.
To ensure the correctness of the resulting generator, $C(v)$ has to be a superset of the neighbors of $v$.
In the following, we discuss different approaches used in the literature to efficiently build the set of candidates $C(v)$.

Von Looz~et~al.~\cite{DBLP:conf/isaac/LoozMP15} shift the problem of generating a random hyperbolic graph to Euclidean space by mapping points into the Poincar\'e disk model.
As a result, neighborhood queries are also mapped onto Euclidean circles.
To gather the set of candidates they then build a polar quad-tree on the Poincar\'e disk and bound the runtime to $\Oh( (n^{3/2} + m) \log n)$ whp.
After generating the quad-tree, edge sampling is trivially parallelizable in a shared memory setting by querying each vertex independently.

Later, von Looz~et~al.~\cite{DBLP:conf/hpec/LoozOLM16} propose a different approach that decomposes the hyperbolic plane into a set of ring-shaped slabs.
They use a set of $k = \Theta(\log n)$ slabs with a geometrically decreasing radial range $[b_j, b_{j+1})$ where $b_j = (1 - \beta^{j-1})R / (1 - \beta^k)$ for $j \in [k{+}1]$ and a tuning parameter~${\beta \approx 0.9}$. 
Each points $(r, \theta)$ is generated randomly within the hyperbolic plane and placed in the corresponding slab~$j$ with $b_j \le r < b_{j+1}$.
Subsequently all points in a slab are sorted order by their angular coordinate.

The candidates $C(v)$ of point $v=(r, \theta)$ in slab $i$ are collected for each $v$ independently by iterating over slabs $i \leq j \leq k$.
In slab $j$ the two angular boundaries $\theta \pm \Delta\theta(r, b_j)$ are computed where $\Delta\theta(r, b_j)$ is obtained based on Eq.~\ref{eq:hypdist} by intersecting the query radius~$R$ with the inner radial boundary~$b_j$ of slab $j$:
\begin{equation}
	\label{eq:deltatheta}
    \Delta\theta(r, b_j) := \cos^{-1}\Big(\frac{\cosh(r)\cosh(b_j) - \cosh(R)}{\sinh(r)\sinh(b_j)}\Big)
\end{equation}
Candidates are then gathered by performing two binary searches (one for each boundary) and iterating over the points between them.
The experimental evaluation of their algorithm suggests a running time of $\Oh(n \log n + m)$.
Furthermore, point and edge sampling can be parallelized easily in a shared memory setting by sampling and querying each point independently.

Bringmann et al.~\cite{DBLP:journals/corr/BringmannKL15} propose a generalization of random hyperbolic graphs named \emph{Geometric Inhomogeneous Random Graphs} (GIRGs).
Additionally, they develop an algorithm to sample GIRGs (and thus RHGs) in expected time $\Oh(n + m)$.
As for the previous approaches, they use a decomposition of the underlying geometric space into discrete cells.
For the case of RHGs, they use a uniform decomposition in the angular direction and an exponential decomposition in the radial direction.
Thus, cells roughly resemble leaves in the quad-tree approach of von Looz et al.~\cite{DBLP:conf/isaac/LoozMP15}.
The main difference is the way they handle neighborhood queries.
Instead of fine-grained queries, they test all point pairs for two related cells in a pessimistic and data-oblivious fashion.
As a consequence, their running time suffers from high constants~\cite{penschuck2017generating}.
A first implementation of their sampling algorithm is provided by Bl\"asius et al.~\cite{DBLP:conf/esa/BlasiusFKL16}.

\Todo{Removed our approaches as discussed via Skype. OK?}
\iffalse
Penschuck~\cite{penschuck2017generating} proposed a memory efficient streaming generator that can be adapted to a distributed setting.
Similar to von Looz et al.~\cite{DBLP:conf/hpec/LoozOLM16}, they partition the hyperbolic plane into concentric slabs.
Vertices in a slab are maintained in sorted order and edges are generated in a request centric approach.
Their algorithm has a memory footprint of $\Oh(n)$ and a running time of $\Oh(n \log \log n + m)$ with high probability.
Futhermore, they present a shared memory parallelization of their algorithm that can be adapted to a distributed setting with a constant communication overhead.
Finally, they present various optimizations for speeding up distance computations.

Recently, Funke et al.~\cite{funke2017communication} presented a communication-efficient distributed graph generator that uses pseudorandomization and divide-and-conquer techniques.
Like previous approaches, they use a decomposition of the hyperbolic plane into slabs.
Similar to Bringmann et al.~\cite{DBLP:journals/corr/BringmannKL15}, each slab is further divided into a set of equidistant buckets.
In contrast to the approaches by von Looz and Penschuck, this allows them to avoid sorting the vertices in each slab.
Thus, they achieve an expected linear running time in the sequential case. 
Additionally, they use pseudorandomization based on hash functions to avoid costly communication in the distributed case in favor for local recomputations.
They continue to show that the expected amount of recomputations is small depending on the power-law exponent.
Finally, they achieve very good scaling behavior even for very large numbers of processors.
\fi


==> hyperbolic/rhg_par.tex <==
In this section, we cover how to adapt our sequential generators for a distributed memory setting.
In particular, we cover how to use pseudorandomization via hash functions to redundantly compute parts of the hyperbolic graph.
This allows us to avoid costly communication between PEs.

\subsection{Threshold Approach}
\label{subsec:par_thres}
As for the sequential generator, we start by decomposing the hyperbolic plane into a set of concentric slabs.
This step is performed by all PEs and synchronized via pseudorandomization;
we compute a unique seed value based on the number of slabs (independent of the rank of the PE).
Afterwards, a (high quality) hash value for this seed is computed and used to initialize a pseudorandom number generator (PRNG) for the multinomial random deviate.
Thus, all PEs compute the same number of vertices for each slab without the need of communication.
\Todo{Why do we need hashing at this point? Is it not more clear (and more versatile) to communicate a seed value with the parameter set that we need to distribute anyways?}

We then add an additional decomposition to our sequential approach by splitting each slab in the angular direction into a set of $k$ equidistant chunks.
These chunks are then evenly distributed among the PEs based on their rank, \ie~PE $i$ is assigned chunks $\lfloor \frac{k}{P} \rfloor \cdot i$ to $\lfloor \frac{k}{P} \rfloor \cdot (i+1)$.
Each PE is then responsible for generating the requests within its set of chunks, processing the corresponding vertices and emitting their incident edges.

To make sure we get the correct distribution of requests to chunks, we use a divide-and-conquer scheme introduced by Sanders~\etal~\cite{sanders2016efficient}.
To be more specific, we begin by splitting the current set of chunks into two evenly sized partitions.
We then determine the number of requests within each partition by computing a binomial random deviate.
Afterwards, each PE follows the partition that contains its local set of chunks.
This process is repeated recursively until each PE is left with its local chunks and their corresponding number of requests.
All of this is done locally, without any need of communication.

To make sure that the distribution of requests to chunks is the same on across all PEs, we again exploit pseudorandomness.
In particular, we compute a unique seed value based on the current recursion subtree at each level of the recursion.
This seed value is then given to a high quality hash function and the result is used to initialize our PRNG for the binomial deviate.
As a result of this, PEs that follow the same recursion subtrees generate the same random deviates, while deviates in different subtrees are independent of each other.
This allows for the generation of consistent deviates without requiring communication.

After we initialized the chunks, each PE continues to divide them further into a set of equidistant buckets as for the sequential approach.
% Figure~\ref{} shows the resulting decomposition of the hyperbolic plane into slabs, chunks and buckets.

Once we finished our decomposition, each PE starts to traverse the slabs outwards as for the sequential approach. \Todo{At lastest here we do need the streaming generation}
However, for the distributed algorithm, the slabs are partitioned into two groups: \emph{lower global slabs} and \emph{upper streaming slabs}.
Global slabs are slabs where the maximum angular deviation of any request is larger than the width of a single chunk $2\pi/p$. 
Likewise, streaming slabs are slabs where the maximum angular deviation of any request is smaller or equal than the width of a single chunk. 

Vertices and requests within the lower global slabs are computed redundantly across all PEs.
In particular, each PE initializes the PRNG for each chunk found in a global slab and then continues to generate the corresponding requests.
Again, consistency across PEs is achieved using pseudorandomness.
The resulting requests are then propagated to a designated buffer in the first upper streaming slab and stored for later use.
Additionally, any requests within a local chunk is output. \Todo{I do not understand what output means.}
As for the sequential approach, requests might get divided into at most two requests depending on their angular deviation.

Due to the nature of hyperbolic space, vertices in the global slabs are likely to have a very high degree since most of these vertices will almost always be within the hyperbolic circle of any vertex.
This can lead to a highly imbalanced workload if we evenly divide the innermost slabs to chunks and assign them to PEs.
To be more specific, if \emph{only} a single chunk contains a very high degree vertex, the associated PE has to generate all edges stemming from the corresponding request.
\Todo{Only for global nodes. Each affected PE in the network will generate a request for such a node and computation of neighbors found during streaming is fully distributed.}
Since the angular deviation of this request is likely to be large for the global slabs, this will lead to a large number of edges and in turn to a significant overhead.
Thus, we designate a small subset of PEs solely to generating the edges for pairs of requests and vertices in the global phase.
For an illustration of the distribution of (global and streaming) slabs and chunks to PEs, we refer to Figure~\ref{fig:hypgen}.

\begin{figure}[t]
  \centering
	{\adjustbox{trim={.24\width} {.4\height} {0.0\width} {.0\height},clip}{
		\scalebox{0.8}{\input{figures/segments.pgf}}
	}}
	\caption{
		The hyperbolic plane is partitioned along the polar axis into $p$ segments of equal size.
		Radially, there are two groups: the lower \emph{global slabs} which are preprocessed and kept in memory, and the upper \emph{streaming slabs}.
		In the main phase, each PE streams through its chunks towards increasing polar angles (red arrow).
		Requests overlapping into the next segment are then completed in the endgame.
  }
	\label{fig:hypgen}
\end{figure}

After we are finished with the global slabs, we then continue with the upper streaming slabs.
As mentioned previously, a PE is only responsible for generating the vertices and requests within its set of local chunks for each of these slabs.
Thus, each PE starts by initializing the PRNG for each of its local chunks in the current slab.
We then iterate over all buckets within the current chunk and generate the corresponding requests and vertices.
All vertices are output and stored (in sorted order) for distance comparisons later on.
Furthermore, each of the requests is added to the state of our sweep line algorithm.
Next, each PE gathers the requests stemming from slabs above the current one.
This includes both requests from the insertion buffer propagated by previous streaming slabs, as well as requests from the global slab buffers.
However, some of these requests will potentially lay outside of the set of local chunks.
We first ignore this problem and only handle the buckets within our local set of chunks.
All remaining requests are processed later in the so-called \emph{endgame} as seen in Figure~\ref{fig:hypgen}.
Finally, each request is propagated to the next slab.

To actually compute the edges resulting from the current set of requests, we iterate over the vertices stored in the current bucket and perform a distance comparisons between the vertices and requests.
Afterwards, we continue with the next bucket.
Since we process buckets in sorted order, we can also remove any request whose angular deviation is smaller than the upper angular boundary of our current bucket.
This allows us to reduce both the number of distance comparisons and memory consumption.
After all buckets are processed, we continue with the next local chunk.
Finally, after all local chunks are finished, we recurse on the next slab.
Once all slabs are processed, we conclude the local phase for the streaming slabs and start the endgame.

For the endgame, each PE is responsible for generating edges that stem from pairs where either the request or vertex stem from the main phase described previously. 
Thus, the endgame can be stopped early once all of these old points are processed.
To do so, we repeat the same process as in the local phase and additionally count the number of remaining old vertices and requests. 

\subsection{Vertices in Global Slabs}
\Todo{%
All Thms start with "If the endgame has a size smaller than the size of a chunk\ldots".
This is true by construction and it seems misleading to repeat it several time in the Thms. What do you think?
Also not "smaller" but "at most".
}


\begin{lemma}\label{lem:global-vertices}
  If the endgame has a size smaller than the size of a chunk and we have $k = \Oh(P)$ chunks, the number of vertices generated in the global slabs is $\Oh(n^{1-\alpha} \bar d^{\alpha} P^{\alpha} + \log n)$ with high probability.
\end{lemma}

\begin{proof}
  Consider the request of a point $(r_G, \delta)$ with an angular deviation of at most $2\Delta\delta(r_G, r_G)$.
  Since we limit the endgame to be smaller than the width of a single chunk, we solve $2\Delta\delta(r_G, r_G) = \frac{2\pi}{k} = \Oh(\frac 1 P)$.
  The number of vertices $n_G(k)$ that each PE has to generate during the global phase is thus binomially distributed around the mean of
\begin{align}
	\expv{n_G(k)} 
    & = n\mu(B_{r_G}(0)) 
     = n \left(\frac{\bar d P}{2n}\right)^\alpha \left(\frac{\alpha - \frac 1 2}{\alpha}\right)^{2\alpha} \\
    & = \Oh\left(n^{1-\alpha} \bar d ^ \alpha P^\alpha \right).
\end{align}
Additionally, for small $(\frac{\bar d}{n})^\alpha$ we add an additional $\Oh(\log n)$ term to ensure concentration.
\end{proof}

\subsection{Vertices in Streaming Slabs}
\begin{lemma}\label{lem:stream-vertices}
  If the endgame has a size smaller than the size of a chunk and we have $k = \Oh(P)$ chunks, the number of vertices generated in the streaming slabs is $\Oh(\frac n P)$ with high probability.
  \Todo{The WHP bound seems wrong in case $P = \Omega(n / \log n)$; did not check it, as I think we should better explicitly bound $P$ somewhere.}
\end{lemma}

\begin{proof}
  We follow the observations used in the proof of Lemma~\ref{lem:global-vertices}.
  Thus, the number of vertices generated in the streaming slabs $n_S(k)$ is binomially distributed around the mean of 
\begin{align}
	\expv{n_S(k)} 
    & = n \mu(B_R(0) \ B_{r_G}(0)) \\
    & = n \left(\frac 2 \pi \cdot \frac{\alpha}{\alpha - \frac 1 2}\right) \left(1 \pm \Oh(1)\right)
\end{align}
  with high probability.
  The claim holds as these vertices are distributed uniformly at random across $\Oh(P)$ chunks.
\end{proof}

\subsection{Edges for Clique PE}
\Todo{What do we use this claim for? Do we wont to say, that the PE responsible for the global graph does not have too much work? In this case, the THM has to be phrased differently not to include the node from the streaming phase.}
\begin{lemma}\label{lem:global-edges}
  If we limit the endgame to the size of a chunk and we have $k=\Oh(P)$ chunks, the number of edges generated for global and clique slabs $m_G(k)$ is $\Oh(n^{2-2\alpha} k^\alpha d^{2\alpha} \log(n))$ with high probability.
\end{lemma}

\begin{proof}
  \Todo{Point $p$ at radius $r$ undefined. I did not add the definition myself since am not sure what the THM will be.}
  Following the proof of Lemma~\ref{lem:neighbors}, we introduce indicator variables $X_1, \ldots, X_n$ with $X_i = 1$ if two points $p$ and $p_i$ are adjacent. 
  This yields the expected value
	\begin{align}
    \expv{X_i} &= 
	\int\limits_{0}^{R-r} \rho(x) \intd x 
	\ \ + \ \ \frac 1 \pi \int\limits_{R-r}^r \rho(x) \Delta\theta(x, R) \intd x \\		
%	&= \left[\e^{-\alpha r} {-} \e^{-\alpha R}\right](1{+}o(1)) +
%	\frac{\alpha}{\pi}\e^{-\alpha R}
%	\int\limits_{R-r}^r \e^{(\alpha-\frac 1 2)x} \left(1 \pm \Oh(e^{-(\alpha +1)x})\right) \intd x\\
  &= \left[\e^{-\alpha r} {-} \e^{-\alpha R}\right](1{+}o(1))  \\ 
  &\phantom{=} + \frac{1}{\pi}\frac{\alpha }{\alpha {-} \frac 1 2}\e^{-\alpha r}
	\left[\e^{(\alpha-\frac 1 2)(2r-R)} - 1\right] (1 \pm \Oh(\e^{-r}))\label{eq:cond-exp-val}
	\end{align}
  To determine the number of neighbors for a vertex in the global slabs, we (pessimistically) assume $r = R/2$.
  This leads to $\expv{X_i} = \Oh((\frac d n)^\alpha)$ and thus an expected number of neighbors $\expv{\Sigma_i X_i} = \Oh(n^{1-\alpha} d^\alpha)$.
  Using a Chernoff bound then yields $\Oh(n^{1-\alpha} d^\alpha)$ neighbors with high probability. \Todo{WHP seems wrong for $\alpha \ge 1$}.
  By combining this result with Lemma~\ref{lem:global-vertices}, we can now bound the number of edges generated in the global slabs by 
\begin{equation}
  m_G(k) = \Oh(n^{2-2\alpha} k^\alpha d^{2\alpha} \log(n))
\end{equation}
  with high probability.
\end{proof}

\subsection{Edges for Streaming PE}
\begin{lemma}\label{lem:stream-edges}
  If we limit the endgame to the size of a chunk and we have $k=\Oh(P)$ chunks, the number of edges generated for streaming slabs $m_S(k)$ is $\Oh((\frac n k)^{2-\alpha} d^\alpha \log(n))$ with high probability.
\end{lemma}

\begin{proof}
  Using the same techniques as in the proof for Lemma~\ref{lem:global-edges}, we are able determine the number of neighbors for a vertex in the streaming slabs.
  For this purpose, we (pessimistically) assume $r = r_G$ (Lemma~\ref{lem:global-vertices}).
  The resulting expected value is given by $\expv{X_i} = \Oh(k^{\alpha - 1} (\frac d n)^\alpha - (\frac d n)^{2 \alpha})$.
  Using a Chernoff bound on $\expv{\Sigma_i X_i}$ then yields $\Oh((\frac n k)^{1-\alpha} d^\alpha \log(n))$ neighbors for each vertex.
  In turn, we can use Lemma~\ref{lem:stream-vertices} to bound the total number of edges for vertices in the streaming bands by 
\begin{equation}
  m_S(k) = \Oh((\frac n k)^{2-\alpha} d^\alpha \log(n))
\end{equation}
  with high probability.

\end{proof}

\subsection{Runtime of Distributed Algorithm}
\begin{theorem}\label{theo:sequential-linear}
\end{theorem}



==> hyperbolic/rhg_seq.tex <==
\Todo{Where do we introduce the streaming part? In the sequential algorithm or the distributed one?
Maybe later is better, as it would require a complete rewrite of this chapter (splitting of requests is not possible anymore, section 3.1 happens interleaved).}

We begin by presenting our sequential generators for the threshold RHG model.
This makes it easier to focus on the main challenges in adapting our algorithms for a distributed setting.  
Nonetheless, most of our observations from this section will naturally translate to the distributed generators.

Similar to existing generators, we begin by performing a geometric decomposition of the hyperbolic plane.
We then use this decomposition in a multi-level sweep line algorithm that emits the vertices and edges of the resulting graph instance in a streaming fashion.

We begin by splitting the hyperbolic plane into a set of concentric slabs with a constant height $x=\lfloor \frac{\alpha R}{\ln 2} \rfloor$, {\ie}
slab~$i$ covers a radial range of $[\ell_i, \ell_{i+1})$ with $\ell_i = i \cdot \lfloor \frac{\alpha R}{\ln 2} \rfloor$.
The particular choice for the slab height~$x$ results in a constant ratio between the expected number of points of two adjacent slabs (see Lemma~\ref{lem:growth-slabs}).
Since all points $(r, \theta)$ with a radius $r \leq R/2$ form a clique, we additionally contract all slabs with an upper boundary $\leq R/2$ into a single slab\Todo{This leads to ambiguity later in the proofs. I suggest, we define $\ell_0=0$, $\ell_1 = R/2$ and $\ell_i = i \cdot \lfloor \frac{\alpha R}{\ln 2} / 2\rfloor$}.
% Figure~\ref{} shows an example of the resulting radial decomposition.

The number of points in each slab are sampled using a multinomial random deviate.
In particular, the probability $p_i$ that a fixed vertex is assigned to slab~$i$ is given by the area of the slab relative to the area of the hyperbolic disk $\mathcal{D}_R$ with radius~$R$:
\begin{equation}
    p_i = \int_{\ell_i}^{\ell_{i+1}} \rho(r) dr = \frac{\cosh(\alpha \cdot \ell_{i+1}) - \cosh(\alpha \cdot \ell_i)}{\cosh(\alpha \cdot R)-1}
\end{equation}

\textsl{
\Todo{Give it a different spin? We use buckets only to get "integer sorting" of requests. Let's call it an optimisation and only describe it, once the alog is clear}
Afterwards, each slab is further partitioned in the angular direction.
This results in a set of $k$ equidistant buckets in each slab.
The number of buckets $k$ is chosen in such a way that each bucket contains an expected constant number of points.
Each of the resulting buckets is then associated with all points within the angular interval $[b_i, b_{i+1})$ with $b_0 = 0$ and $b_i = i \cdot \lfloor \frac{2\pi}{k} \rfloor$.
As for the slabs, we use a multinomial random deviate to determine the number of vertices in each bucket.\Todo{Why? It's not necessary in the sequential case if we draw increasing $\theta$'s.}
Since points are distributed uniformly in the angular direction, the probability that a vertex is assigned bucket $j$ in slab $i$ simply is $p_{i, j} = \frac{n \cdot p_i} k$.}

\textsl{
Points within a slab are generated in increasing order of their angular coordinate.
Thus, each bucket only needs to store its first associated point and the number of points it contains.
In addition to the points themselves, each bucket also maintains a set of \emph{requests} for buckets lying in a lower (or the same) slab.
Each request $\text{req}_{i,j}(p)$ for a point $p$ (stored in slab $i$ and bucket $j$) is composed of its coordinates $(r, \theta)$, as well as the angular deviation \Todo{(more verbose: request width?)} of neighbors within slab $i$.
By using this request-centric approach, we can drastically reduce the number of random accesses during candidate selection and carry precomputed values repeatedly used by distance calculations.}


\Todo{This paragraph has some redundancy compared to the previous one; also we do not sample the vertices but the beginning of the requests and then place the vertex. This is very crucial to get dependencies right.}
After computing the partitioning of the hyperbolic plane into slabs and buckets, our generator traverses the slabs outwards starting with the innermost slab.
This traversal represents the first level of our sweep line algorithm.
Within each slab, we begin by generating the associated vertices in increasing order of their angular coordinate using the sampling approach of Bentley and Saxe~\cite{DBLP:journals/toms/BentleyS80}.
During the generation of a vertex we also build the corresponding request.
This includes computing a set of values that allow us to speed-up frequent distance calculations, as well as the angular deviation of neighbors within the current slab.
Each request is then added to an insertion buffer for the current slab.

During the creation of a request, it might happen that we encounter an angular deviation of $[a,b]$ where either $a < 0$ or $b > 2\pi$ (or both) \Todo{how can it be both? Any request has length $\le 2\pi$ or did I miss something?}.
Taking the angular $2\pi$-period of the hyperbolic plane into account, these requests are separated into two ranges.
To be more specific, we separate the angular deviation $[a,b]$ with $a<0$ into the two ranges $[a + 2\pi, 0]$ and $[0,b]$.
The case $b>2\pi$ is treated analogously.
In case both $a<0$ and $b>2\pi$, we insert a single request with a angular deviation of $[0,2\pi]$.

\subsection{Threshold Approach}
After we generated all vertices and requests, we distribute each request to the first bucket (in terms of the lower angular boundaries) that lies within the range $[a,b]$.
This process can be done in linear time using sample sort~\cite{}.
We then continue to scan each bucket containing at least one request which represents the second level of our sweep line algorithm.

\Todo{I do not understand the paragraph}
To avoid iterating over empty buckets, we maintain the smallest and largest angular deviation for the current slab.
Each bucket within the range defined by these deviation is then guaranteed to yield at least a single request.

Next, we compare the angular deviation of a request with the vertices contained in the current bucket.
We do so by processing vertices in increasing order of their angular coordinate, and comparing them to the set of remaining requests.
Thus, each vertex serves as an event for the final level of our sweep line approach.
For an overview of the individual sweep line procedures, see Figure~\ref{fig:sweep}.

\begin{figure}[t]
  \centering
  \includegraphics[scale=0.7]{figures/sweepline_levels.pdf}
	\caption{
    Overview of the different sweep line algorithms used in our threshold generator.
		\textbf{Left}: First outward sweep performed over the constant height slabs.
		\textbf{Middle}: Second sweep over the equidistant buckets that have at least one request in each slab.
		\textbf{Right}: Third sweep over all vertices in increasing angular direction within the current bucket.
    The current slab, buckets and vertices are highlighted in blue.
	}
	\label{fig:sweep}
	\vspace{-1em}
\end{figure}

If a vertex lies within the angular range of a request, we perform a distance computation using the precomputed values associated with the request.
The result of this computation then may yield an edge of our resulting graph.
Likewise, if a vertex lies outside the request range, the request is dropped from the bucket, since we can be sure that all further vertices also lie outside the range.
This approach allows us to greatly reduce the number of comparisons within a single bucket. \Todo{The implementation does not do this; as it contradicts the point of having the buckets. This also gives us only a $\ll 2$ factor, since the symmetric case at the beginning of the bucket cannot be fixed this way.}

If a request is dropped from a bucket, we propagate it to the next slab by updating its angular deviation and adding it to the corresponding insertion buffer. \Todo{In the streaming setting we propagate it as soon as the lower requests becomes active! Otherwise we cannot jump to the next higher slab.}
Otherwise, if a set of requests is not dropped after processing the current bucket, we move them to the next bucket.
We then repeat this procedure until we reach the first empty bucket.
After all requests have been processed we move our sweep line to the next slab.
 
\subsection{Decomposition has Constant Growth Factor}
In this section, we show that our decomposition of the hyperbolic plane results in a constant growth factor for the number of vertices in successive slabs.

\begin{lemma}\label{lem:growth-slabs}
The number of vertices between successive slabs with a lower radial boundary $\geq R/2$ grows by a constant factor at worst.
In particular, the expected number of vertices $n_i$ in a slab with an upper radial boundary of $b_i = i \cdot \lfloor \frac{\ln 2}{\alpha} \rfloor$ is $n_i = 2^i n e^{-\alpha R} (1+o(1))$.

\Todo{Has inner most slab height $R/2$?}
\end{lemma}

\begin{proof}
  The probability mass of a slab $i$ with an upper radial boundary $b_{i + 1}= (i + 1) \cdot \lfloor \frac{\ln 2}{\alpha} \rfloor$ is given by the cdf
\begin{align*}
  \mu(B_{b_{i+1}}(0)) - \mu(B_{b_i}(0)) = 2^ie^{-\alpha R}(1+o(1)). & \tag*{(Eq.~\ref{eq:cdf})}
\end{align*}
  In particular, the probability mass of the innermost slab with an upper radial boundary of $b_1 = \lfloor \frac{\ln 2}{\alpha} \rfloor$ is
\begin{align*}
  \mu(B_{b_1}(0)) &= e^{\alpha (b_0-R)}(1+o(1))\\
                  & = \frac{2}{e^{\alpha R}}(1+o(1)).
\end{align*}

  In turn, the ratio between the probability masses of two successive slabs is 
\begin{align*}
 \frac{\mu(B_{b_{i+1}}(0))}{\mu(B_{b_i}(0))} 
 \stackrel{(i)}{=} \frac{\cosh(\alpha \ell_{i+1})}{\cosh(\alpha \ell_i)}
 \stackrel{(ii)}{=} \frac{2e^{\alpha \ell_i} + e^{-\alpha \ell_i}/2}{e^{\alpha \ell_i} + e^{-\alpha  \ell_i}} \le 2
\end{align*}
	In step~(i) we used Eq.~\ref{eq:cdf}, in step~(ii) we substitute $\ell_{i+1} = \ell_i + \ln2/\alpha$ and $\cosh(x) = (e^x + e^{-x}) / 2$.

  Thus, the expected value for the number of vertices in slab $i$ is $n_i = n\mu(B_{b_i}(0)) = 2^i n e^{-\alpha R} (1+o(1))$.
\end{proof}

\subsection{Candidate Selection is Constant Approximation}

\begin{lemma}\label{lem:candidates}
	Consider a query point with radius $r$ and a slab with boundaries $[a, b)$.
	Our candidate selection overestimates the probability mass of the actual query range by a factor of $OE(b{-}a, \alpha)$ where $OE(x,\alpha) \defrel \frac{\alpha - 1/2}{\alpha} \frac{1 - \e^{\alpha x}}{1 - \e^{(\alpha-1/2)x}}$.%(1 + O(\e^{(\alpha-1/2)(R-2a-r)}))$.
\end{lemma}

\begin{proof}
	If $r < R{-}b$, the requesting point covers the slab completely which renders the candidate selection process optimal.
	We now consider $r \ge R{-}a$ and omit the fringe case of $R{-}b < r < R{-}a$ which follows analogously (and by continuity between the two other cases).
	Then, the probability mass $\mu_Q$ of the intersection of the actual query circle $B_R(r)$ with the slab $B_b(0) \setminus B_a(0)$ (cf. Fig.~\ref{fig:hyperbolic_model}, blue cover of a slab) is given by
  \begin{align*}
    \mu_Q &\defrel \mu\left[ (B_b(0) {\setminus} B_a(0)) \cap B_R(r) \right] \\
		&\stackrel{\phantom{(\ref{eq:muupper})}}{=} \frac 2 \pi \e^{-\frac r 2 - (\alpha-\frac 12)R} \cdot \\
    &\phantom{==} \left[
		\frac{\alpha}{\alpha{-}\frac 1 2}\left(
		\e^{(\alpha-\frac 1 2)b} - \e^{(\alpha-\frac 1 2)a}
		\right)
		+ \errorterm{\Oh\left(\e^{-(\alpha{-}\frac 1 2)a}\right)}
		\right],
  \end{align*}
	
	Our generator overestimates the actual query range at the border and covers the mass $\mu_H$ (see Fig.~\ref{fig:hyperbolic_model}, yellow cover of a slab):
  \begin{align*}
		\mu_H &\defrel \frac 1 \pi \Delta\theta(r, a) \int\limits_a^b \rho(y) dy \\
      &=\frac 2 \pi \e^{-\frac r 2 - (\alpha-\frac 12)R} \cdot \\
      &\phantom{=} \left[ 
		\e^{\alpha b - a/2} - \e^{(\alpha - \frac 12)a}
		\right] \cdot \errorterm{\left(1 \pm \Oh\left(\e^{(1-\alpha)(R-a)-r}\right)\right)}.
  \end{align*}
	
	The claim follows by the division of both mass functions  ${\mu_H}/{\mu_Q}$.
\end{proof}

\begin{corollary}\label{cor:candidates}
	Given a constant slab height, i.e. $b{-}a=\Oh(1)$, Lemma~\ref{lem:candidates} implies a constant overestimation for any $\alpha {>} 1/2$.
  In case of $b{-}a=\lfloor \frac{\ln(2)}{\alpha} \rfloor$, we have $OE(1, \alpha) \le \sqrt{\e} \approx 1.64 \ \ \forall \alpha{>}1/2$.
\end{corollary}

\subsection{Bounding the Number of Neighbors}
\begin{lemma}\label{lem:neighbors}
	Let $N_j$ be the number of neighbours the point $p_j {=} (r_j, \theta_j)$ has from below, i.e. neighbours with smaller radius.
	With high probability, there exist $\Oh(n / \log^2 n)$ points with $N_j = \Oh(n^{1-\alpha} \bar d ^ \alpha  \log(n))$ while the remainder of points with $r_j > R/2$ has $N_j = \Oh(n^{1 - 2\alpha}\log^{2\alpha}(n) \bar d ^ {2\alpha})$ neighbours.
\end{lemma}

\begin{proof}
	Let $X_1, \ldots, X_n$ be indicator variables with $X_i {=} 1$ if $p$ and $p_i$ are adjacent.
	Due to radial symmetry we directly obtain the expectation value of $X_i$ conditioned on the radius $p_i$:
	\begin{align}
    \expv{X_i\ |\ r_i{=x}} & = \prob{X_i {=} 1\ |\ r_i{=x}} \\
                         & = \begin{cases}
		1 & \text{if } x < R - r \\		
		\Delta\theta(x, r) / \pi & \text{otherwise}
		\end{cases} 
	\end{align}
	
	\noindent We remove the conditional using the Law of Total Expectation and equations (\ref{eq:deltathetaapprox}) and (\ref{eq:cdf}):
	\begin{align}
    \expv{X_i} &= 
	\int\limits_{0}^{R-r} \rho(x) \intd x 
	\ \ + \ \ \frac 1 \pi \int\limits_{R-r}^r \rho(x) \Delta\theta(x, R) \intd x \\		
%	&= \left[\e^{-\alpha r} {-} \e^{-\alpha R}\right](1{+}o(1)) +
%	\frac{\alpha}{\pi}\e^{-\alpha R}
%	\int\limits_{R-r}^r \e^{(\alpha-\frac 1 2)x} \left(1 \pm \Oh(e^{-(\alpha +1)x})\right) \intd x\\
  &= \left[\e^{-\alpha r} {-} \e^{-\alpha R}\right](1{+}o(1))  \\ 
  &\phantom{=} + \frac{1}{\pi}\frac{\alpha }{\alpha {-} \frac 1 2}\e^{-\alpha r}
	\left[\e^{(\alpha-\frac 1 2)(2r-R)} - 1\right] (1 \pm \Oh(\e^{-r}))\label{eq:cond-exp-val}
	\end{align}
	
	\noindent
	Fix the radius $r_T  =  R {-} \frac 2 \alpha \log\log n$ with $R/2 < r_T$ (wlog) and consider three cases for $r$:
  First, we ignore all points $r \le R/2$ as they belong to the central clique and are irrelevant here.
  Second, observe that with high probability there exist $\Oh(n / \log^2(n))$ points below $r_T$. 
  Exploiting the monotonicity of Eq.~\ref{eq:cond-exp-val} in $r$, we maximise it by setting $r = R/2$, which cancels out the second term.
  Linearity of the expectation value, substitution of $R = 2\log(n) + C$, and Eq.~(\ref{eq:exp-deg}) yield
%			\begin{align}
$				\expv{\sum_i X_i} 
%				&= n \expv{X_1} 
%				= n \left[\e^{-\frac \alpha 2 R} - \e^{-\alpha R}\right] (1 + o(1)) \\
%				&= n \left[n^{-\alpha} \e^{-\alpha C} - n^{-2\alpha}\e^{-\alpha C}\right] (1 + o(1)) \\
%				&= n^{1-\alpha} \bar d^\alpha 
%				\left(\frac \pi 2 \right)^{\alpha}
%				\left(\frac{\alpha - \frac 1 2}{\alpha}\right)^{2\alpha}
%				(1 + \Oh(n^{-\alpha}k^\alpha))
				= \Oh\left[n \left({\bar d}/{n} \right)^\alpha \right]  
%			\end{align}
$.
  Then, Chernoff's bound gives $\sum_i X_i = \Oh(n^{1-\alpha} \bar d ^ \alpha  \log(n))$ with high probability.
	Third, for all points above $r_T$, set $r = r_T$ yielding $\sum_i X_i = \Oh(n^{1 - 2\alpha}\log^{2\alpha}(n) \bar d ^ {2\alpha})$ with high probability analogously.
\end{proof}



\subsection{Linear Runtime of Sequential Algorithm}

\begin{theorem}\label{theo:sequential-rt}
  \rhgthres requires $\Oh(n)$ memory and has a runtime of $\Oh(n \log \bar d + m)$ with high probability.
\end{theorem}


\begin{proof}
	The space complexity directly follows from Alg.~\ref{alg:memgen}: 
	each of the $n$ points is stored in exactly one slab, yields at most two requests, and requires $\Oh(1)$ space in the candidate list.
	During the main phase, there further exists only one insertions buffer at a time to which a point may contribute $\Oh(1)$ items.
	\hfill
	
	\noindent We bound \rhgthres's time complexity by considering each component individually:
	\begin{itemize}
		\item The preprocessing requires $\Oh(1)$ time per point making it non-substantial.
		\item Handling of cliques is trivially bounded by $\Oh(m)$ since every iteration emits an edge.
		\item Processing the requests within the bucket requires $\Oh(n)$ time in total with high probability according to Lemma~\ref{lem:bucket-requests}
		\item By applying Lemma~\ref{lem:neighbors} and Cor.~\ref{cor:candidates}, the candidate selection requires $\Oh(n\log \bar d)$ time with high probability.
		\item All distance calculations require in total $\Oh(m)$ time since Cor.~\ref{cor:candidates} bounds the fraction of computations that do not yield an edge to $\Oh(1)$.
	\end{itemize}
	\vspace{-1em}
\end{proof}


==> hyperbolic/rhg_thres.tex <==
We begin by presenting our sequential generators for the threshold and probabilistic RHG model.
For this purpose, we mainly focus on presenting our memory efficient implementations and analyzing their sequential running time.
This makes it easier to focus on the main challenges in adapting our algorithms for a distributed setting.  
Nonetheless, most of our observations from this section will naturally translate to the distributed generators.

Similar to existing generators, we begin by performing a geometric decomposition of the hyperbolic plane.
We then use this decomposition for developing a multi-level sweep-line algorithm that emits the vertices and edges of the resulting graph instance.

We begin our decomposition by splitting the hyperbolic plane into a set of concentric annuli with a constant height $x=\lfloor \frac{\alpha R}{\ln 2} \rfloor$.
Thus, annulus\todo{Consistency slabs or annuli but not both?} $i$ covers a radial range of $[l_i, l_{i+1})$ with $l_0 = 0$ and $l_i = i \cdot \lfloor \frac{\alpha R}{\ln 2} \rfloor$.
The particular choice for the annulus height is motivated by ensuring a constant growth factor for the number of points in consecutive annuli (see Lemma~\ref{}).

Since all points $(\phi, r)$\todo{Consistency -- in section 2 it's $(r, \phi)$} with a radius $r \leq R/2$ form a clique, we additionally contract all annuli with an upper boundary $\leq R/2$ into a single annulus.
Figure~\ref{} shows an example of the resulting radial decomposition.

Computing the number of points in each annulus can be done by using a multinomial random deviate.
The probability $p_i$ that a vertex is assigned a particular annulus $i$ is given by the quotient of the area of the annulus and the area of the hyperbolic disk with radius $R$.
To be more specific, \todo{Consistency: Earlier it's $f()$ is called $\rho$}
\begin{equation}
    p_i = \int_{r_i}^{r_{i+1}} f(r) dr = \frac{\cosh(\alpha \cdot r_{i+1}) - \cosh(\alpha \cdot r_i)}{\cosh(\alpha R)-1}.
\end{equation}

We then perform a second partitioning within each annulus in the angular direction.
We do so by splitting each annulus into a set of $k$ equidistant buckets.
The number of buckets $k$ is chosen in such a way that each bucket contains an expected constant number of points.
Again, each bucket contains all points within the corresponding interval $[b_i, b_{i+1})$ with $b_0 = 0$ and $b_i = i \cdot \lfloor \frac{2\pi}{k} \rfloor$.
As before, we use a multinomial random deviate to determine the nuber of vertices in each bucket.\todo{Why? It's not necessary in the sequential case if we draw increasing $\phi$'s.}\todo{Buckets or cells?}
Since points are distributed uniformly in the angular direction, the probability that a vertex is assigned bucket $j$ in annulus $i$ simply is $p_{i, j} = \frac{n \cdot p_i} k$.

Points within an annulus are generated in increasing order of their angular coordinate.
Thus, each bucket only needs to store its first associated point and the number of points it contains.
In addition to the points themselves, each bucket also maintains a set of \emph{requests} for buckets lying in a lower (or the same) annulus.
Each request $\text{req}_{i,j}(p)$ for a point $p$ (stored in annulus $i$ and bucket $j$) is composed of its coordinates $(\phi, r)$, as well as the angular deviation of neighbors within annulus $i$.
By using this request-centric approach, we can drastically reduce the number of random accesses during candidate selection and carry precomputed values repeatedly used by distance calculations.

After computing the partitioning of the hyperbolic plane into annuli and buckets, our generator traverses the annuli outwards starting with the innermost annulus.
This traversal represents the first level of our sweep-line algorithm.
Within each annulus, we begin by generating the associated vertices in increasing order of their angular coordinate using the sampling approach of Bentley and Saxe~\cite{DBLP:journals/toms/BentleyS80}.
During the generation of a vertex we also build the corresponding request.
This includes computing a set of values that allow us to speed-up frequent distance calculations, as well as the angular deviation of neighbors within the current annulus.
Each request is then added to a insertion buffer for the current annulus.

During the creation of a request, it might happen that we encounter an angular deviation of $[a,b]$ where either $a < 0$ or $b > 2\pi$ (or both).
Taking the azimuthal $2\pi$-period of the hyperbolic plane into account, these requests are separated into two ranges.
To be more specific, we separate the angular deviation $[a,b]$ with $a<0$ into the two ranges $[a + 2\pi, 0]$ and $[0,b]$.
The case $b>2\pi$ is treated analogously.
In case both $a<0$ and $b>2\pi$, we insert a single request with a angular deviation of $[0,2\pi]$.

The processing of request within an annulus is governed by the way edges are computed which depends on the underlying graph model (threshold or probabilistic).
We now describe how we handle request in the threshold RHG model and then generalize our results for the probabilistic case.

\subsection{Threshold approach}
After all vertices and requests have been generated, we distribute each requests to the first bucket that lies within the range $[a,b]$ given by its angular deviation.
This process can be done in linear time using sample sort~\cite{}.
We then continue to scan each bucket containing at least one request which represents the second level of our sweep-line algorithm.

To avoid iterating over empty buckets, we maintain the smallest and largest angular deviation for the current annulus.
Each bucket within this range is then guaranteed to yield at least a single request.

Next, we compare the angular deviation of a request with the vertices contained in the current bucket.
We do so by processing vertices in increasing order of their angular coordinate, and comparing them to the set of remaining requests.
Thus, each vertex serves as an event for the final level of our sweep-line approach.

If a vertex lies within the angular range of a request, we perform a distance computation using the precomputed values associated with the request.
The result of this computation then may yield an edge of our resulting graph.
Likewise, if a vertex lies outside the request range, the request is dropped from the bucket, since we can be sure that all further vertices also lie outside the range.
This approach allows us to greatly reduce the number of comparisons within a single bucket.

If a request is dropped fom a bucket, we propagate it to the next annulus by updating its angular deviation and adding it to the corresponding insertion buffer.
Otherwise, if a set of requests is not dropped after processing the current bucket, we move them to the next bucket in the angular direction.
Afterwards, we repeat this procedure until we reach the first empty bucket.
We can then move our sweep-line to the next annulus, until we processed the complete hyperbolic disk.

\subsection{Decomposition has constant growth factor}
In this section, we show that our decomposition of the hyperbolic plane results in a constant growth factor for the number of vertices in successive annuli.

\begin{lemma}\label{lem:growth-bands}
The number of vertices between successive annuli with a lower radial boundary $\geq R/2$ grows by a constant factor at worst.
In particular, the number of vertices $n_i$ in an annulus with an upper radial boundary of $b_i = i \cdot \lfloor \frac{\ln 2}{\alpha} \rfloor$ is $n_i = 2^i n e^{-\alpha R} (1+o(1))$ with high probability.
\end{lemma}

\begin{proof}
  The probability mass of an annulus $i$ with an upper radial boundary $b_{i + 1}= (i + 1) \cdot \lfloor \frac{\ln 2}{\alpha} \rfloor$ is given by the cdf
\begin{align*}
  \mu(B_{b_{i+1}}(0)) - \mu(B_{b_i}(0)) = 2^ie^{-\alpha R}(1+o(1)). & \tag*{(Eq.~\ref{eq:cdf})}
\end{align*}
  In particular, the probability mass of the innermost annulus with an upper radial boundary of $b_1 = \lfloor \frac{\ln 2}{\alpha} \rfloor$ is
\begin{align*}
  \mu(B_{b_1}(0)) &= e^{\alpha (b_0-R)}(1+o(1))\\
                  & = \frac{2}{e^{\alpha R}}(1+o(1)).
\end{align*}

  In turn, the ratio between the probability masses of two successive annuli is 
\begin{align*}
  \frac{\mu(B_{b_{i+1}}(0))}{\mu(B_{b_i}(0))} = \frac{e^{\alpha (b_{i+1}-R)}(1+o(1))}{e^{\alpha (b_i-R)}(1+o(1))} = 2.
\end{align*}

  Using this result, the probability mass of annulus $i$ is given by $\mu(B_{b_i}(0))= \frac{2^{i+1}}{e^{\alpha R}} (1+o(1))$.
  We then get the probability mass for number of vertices in annulus $i$ by $n_i = n\mu(B_{b_i}(0))$.
\end{proof}

\subsection{Bucket contains constant number of vertices}

\begin{lemma}\label{lem:bucket-vertices}
\end{lemma}

\begin{proof}
\end{proof}
\subsection{Candidate selection is constant approximation}

\begin{lemma}\label{lem:candidates}
	Consider a query point with radius $r$ and an annulus with boundaries $[a, b)$.
	Our candidate selection overestimates the probability mass of the actual query range by a factor of $OE(b{-}a, \alpha)$ where $OE(x,\alpha) \defrel \frac{\alpha - 1/2}{\alpha} \frac{1 - \e^{\alpha x}}{1 - \e^{(\alpha-1/2)x}}$.%(1 + O(\e^{(\alpha-1/2)(R-2a-r)}))$.
\end{lemma}

\begin{proof}
	If $r < R{-}b$, the requesting point covers the annulus completely which renders the candidate selection process optimal.
	We now consider $r \ge R{-}a$ and omit the fringe case of $R{-}b < r < R{-}a$ which follows analogously (and by continuity between the two other cases).
	Then, the probability mass $\mu_Q$ of the intersection of the actual query circle $B_R(r)$ with the annulus $B_b(0) \setminus B_a(0)$ (cf. Fig.~\ref{fig:hyperbolic_model}, blue cover of an annulus) is given by
  \begin{align*}
    \mu_Q &\defrel \mu\left[ (B_b(0) {\setminus} B_a(0)) \cap B_R(r) \right] \\
		&\stackrel{\phantom{(\ref{eq:muupper})}}{=} \frac 2 \pi \e^{-\frac r 2 - (\alpha-\frac 12)R} \cdot \\
    &\phantom{==} \left[
		\frac{\alpha}{\alpha{-}\frac 1 2}\left(
		\e^{(\alpha-\frac 1 2)b} - \e^{(\alpha-\frac 1 2)a}
		\right)
		+ \errorterm{\Oh\left(\e^{-(\alpha{-}\frac 1 2)a}\right)}
		\right],
  \end{align*}
	
	Our generator overestimates the actual query range at the border and covers the mass $\mu_H$ (see Fig.~\ref{fig:hyperbolic_model}, yellow cover of an annulus):
  \begin{align*}
		\mu_H &\defrel \frac 1 \pi \Delta\theta(r, a) \int\limits_a^b \rho(y) dy \\
      &=\frac 2 \pi \e^{-\frac r 2 - (\alpha-\frac 12)R} \cdot \\
      &\phantom{==} \left[ 
		\e^{\alpha b - a/2} - \e^{(\alpha - \frac 12)a}
		\right] \cdot \errorterm{\left(1 \pm \Oh\left(\e^{(1-\alpha)(R-a)-r}\right)\right)}.
  \end{align*}
	
	The claim follows by the division of both mass functions  ${\mu_H}/{\mu_Q}$.
\end{proof}

\begin{corollary}\label{cor:candidates}
	Given a constant annulus height, i.e. $b{-}a=\Oh(1)$, Lemma~\ref{lem:candidates} implies a constant overestimation for any $\alpha {>} 1/2$.
  In case of $b{-}a=\lfloor \frac{\ln(2)}{\alpha} \rfloor$, we have $OE(1, \alpha) \le \sqrt{\e} \approx 1.64 \ \ \forall \alpha{>}1/2$.
\end{corollary}

\subsection{Probabilistic approach}

